Streaming Tensor Train Approximation

Tensor trains are a versatile tool to compress and work with high-dimensional data and functions. In this work we introduce the Streaming Tensor Train Approximation (STTA), a new class of algorithms for approximating a given tensor $\mathcal T$ in the tensor train format. STTA accesses $\mathcal T$ exclusively via two-sided random sketches of the original data, making it streamable and easy to implement in parallel -- unlike existing deterministic and randomized tensor train approximations. This property also allows STTA to conveniently leverage structure in $\mathcal T$, such as sparsity and various low-rank tensor formats, as well as linear combinations thereof. When Gaussian random matrices are used for sketching, STTA is admissible to an analysis that builds and extends upon existing results on the generalized Nystr\"om approximation for matrices. Our results show that STTA can be expected to attain a nearly optimal approximation error if the sizes of the sketches are suitably chosen. A range of numerical experiments illustrates the performance of STTA compared to existing deterministic and randomized approaches.

==> OTTS.tex <==
\section{Orthogonalized TT-sketch (OTTS)}

\textcolor{red}{??? Suggestion to be checked: Similar to Daas et al. (?), can exploit nestedness. But not a good idea for parallel-in-mode. ???}

\textcolor{red}{??? Say differently: Oblique projectors lead to additional constants in theorem, blabla. Can be avoided with by a modification ???}

In this section, we explain how to modify the STTA algorithm to improve the quality of the approximation at the expense of losing
the streaming capability and some available parallelism. The difference to STTA is twofold. First, instead of
sketching on the left with $Y_{\mu-1}$ when forming $\Psi_\mu$, we sketch with $C_{\leq \mu-1}$, the
partial contraction from $1$ to $\mu-1$ of the cores of the TT approximation obtained thus far:
% \begin{figure}[htb]
%   \centering
%   \includegraphics[]{images/sketch-orthogonal.pdf}
% %   \caption{Graphical summary of the orthogonalized TT-sketch algorithm.}\label{fig:orthogonal-sketch-summary}
% \end{figure}

\begin{ceqn}
\begin{equation}\label{eq:diagram_def_OTTS_Psi_mu}
\begin{matrix}
\includegraphics{sketch-orthogonal.pdf}
\end{matrix}
\end{equation}
\end{ceqn}

Furthermore, after forming the core
$C_\mu$, we perform an additional orthogonalization step. The procedure is detailed in
\cref{alg:orth-sketch}. 
%The computation of the sketch $\Psi_\mu$ is explained graphically in \cref{fig:orthogonal-sketch-summary}.



\begin{algorithm}
  \caption{OTTS: \texttt{sketch \& assemble}}\label{alg:orth-sketch}
  \begin{algorithmic}[1]
    \REQUIRE Tensor $\mathcal T$ of shape $n_1\times \dots \times n_d$; Left DRM ranks $(r_1^L,\dots,r_{d-1}^L)$; Right DRM ranks $(r_1^R,\dots,r_{d-1}^R)$.
    \ENSURE Cores $C_\mu$ of shape $r_{\mu-1}^L\times n_\mu\times r_\mu^L$ for $1\leq \mu\leq d$ of a tensor train approximation of $\mc T$.
    
    \FOR{$\mu=1$ to $d-1$}
    \STATE Generate DRM $X_\mu$ of shape $(n_{\mu+1} \cdots n_d) \times r_\mu^R$
    \STATE Generate DRM $Y_\mu$ of shape $(n_1\cdots n_\mu) \times r_\mu^L$ 
    \ENDFOR

    \FOR{$\mu=1$ to $d$}
    \STATE $\mathcal T^{\leq \mu} \leftarrow \mathtt{reshape}(\mathcal T,\, (n_1\cdots n_\mu) \times (n_{\mu+1}\cdots n_d))$
    \IF{$\mu=1$}
      \STATE $\Psi_1 \leftarrow \mathcal T^{\leq 1}X_1$
      \ELSIF{$\mu<d$}
    \STATE $\Psi_\mu \leftarrow (C_{\leq \mu-1}^\top\tensor I_{n_\mu}) \mathcal T^{\leq \mu} X_\mu$
    \ELSE
    \STATE $\Psi_d \leftarrow (C_{\leq d-1}^\top\tensor I_{n_d}) \mathcal T^{\leq d}$
    \ENDIF
    \IF{$\mu<d$}
    \STATE $\Omega_\mu \leftarrow Y_\mu^\top \mathcal T^{\leq \mu} X_\mu$
    \STATE $B_\mu^L \leftarrow \mathtt{lstsq}(\Omega_\mu^\top,\,(\Psi_\mu^L)^\top)^\top$\hfill // Stable least-square solver for $B_\mu^L=\Psi_\mu^L \Omega_\mu^\dagger$ as in \cref{eq:Cmu-as-lstsq}
    \STATE $C_\mu^L \leftarrow \mathtt{orth}(B_\mu^L)$ \hfill // Q factor of QR decomposition
    \STATE $C_{\leq \mu}\leftarrow (C_{\leq \mu-1}\otimes I_{n_{\mu}})C_\mu^L$ \hfill // Not formed explicitly
    \STATE $C_\mu \leftarrow \mathtt{reshape}(C_\mu^L,\,r_{\mu-1}^L\times n_\mu \times r_\mu^L)$
    \ELSE
    \STATE $C_d\leftarrow \Psi_d$
    \ENDIF
    \ENDFOR
  \end{algorithmic}
\end{algorithm}



If we use TT DRMs as in \cref{def:tt-drm}, then the computational cost of \cref{alg:orth-sketch} is almost identical to that of STTA in \cref{alg:sketch,alg:assemble}. In particular, it can be applied efficiently to the same class of structured tensors as for SSTA. The only difference in cost is the orthogonalization of the cores $C_\mu$, which is $O(r^3n)$ flops. We also observe that while OTTS does not support streaming, the sketches $\Omega_\mu$ and $\Psi_\mu$ are still linear in the input tensor $\mc T$ for a fixed $\mu$. Therefore, it is still possible to efficiently sketch linear combinations of tensors with OTTS but not in a streaming fashion for all $\mu$ independently.

 \textcolor{red}{BV: Difference to HTM for TT-SVD? Is it only steps 15-17 where $Y_\mu$ takes the role of a q factor of $\Psi_\mu$}
 
When using Gaussian DRMs as in \cref{def:gaussian-drm}, the approximation error of OTTS is also comparable to that of STTA but is in general lower. This is clearly reflected in our numerical experiments from \cref{sec:numerical-experiments} and it also follows from the theoretical upper bound. To analyze the error, we first need the following lemma.

\textcolor{red}{??? Add some intuition ???}

\newcommand{\orthproj}{\mathit{\Pi}\kern-1pt}
\begin{lemma}\label[lemma]{lem:projector-inequality}
%   Let ${\orthproj}$ be an $m\times m$ orthogonal projector, and let $M$ be an $m\times n$ matrix such that ${\orthproj}$ has full rank $n$ with $m \ge n$. Finally let $Y$ be any $n\times m$ matrix. Then
Let ${\orthproj}$ be an orthogonal projector and let $M$ be a matrix such that ${\orthproj} M$ has full column rank. Then for any matrix $Y$ of the same size as $M$ it holds
  \begin{equation}\label{eq:proj_id_PM_with_Y}
    {\orthproj}-{\orthproj} M({\orthproj} M)^\dagger = {\orthproj}(I-{\orthproj} M({\orthproj} M)^\dagger)(I-MY^\top).
  \end{equation}
  In addition, for any matrix $A$ it holds
  \begin{equation}\label{eq:proj_bound_PM_with_A}
    \|{\orthproj} A-{\orthproj} M({\orthproj} M)^\dagger A\|_F \leq \|A-MY^\top\!A\|_F.
  \end{equation}
\end{lemma}
\begin{proof}
Let ${\orthproj}M$ be an $m \times n$ matrix. By assumption $\rank({\orthproj}M) =n$, which implies $m \geq n$ and thus
  \[
    ({\orthproj} M)^\dagger M = (M^\top {\orthproj} M)^{-1} M^\top{\orthproj} M = I_n.
  \]
  Since ${\orthproj} M({\orthproj} M)^\dagger MY^\top$ is an $m\times m$ matrix, it is of the same size as ${\orthproj}$ and ${\orthproj} M({\orthproj} M)^\dagger$. We therefore have with the identity above that
  \begin{align*}
    {\orthproj} - {\orthproj} M({\orthproj} M)^\dagger &= {\orthproj} -{\orthproj} M({\orthproj} M)^\dagger MY^\top+{\orthproj} M({\orthproj} M)^\dagger MY^\top - {\orthproj} M({\orthproj} M)^\dagger \\
    &={\orthproj}(I_m-M I_n Y^\top)-{\orthproj}({\orthproj} M ({\orthproj} M)^\dagger (I_m-MY^\top))\\
    &={\orthproj}(I_m-{\orthproj} M({\orthproj} M)^\dagger)(I_m-MY^\top)
  \end{align*}
  The bound~\eqref{eq:proj_bound_PM_with_A} follows from~\eqref{eq:proj_id_PM_with_Y} and the fact that ${\orthproj}$ and $I-{\orthproj} M({\orthproj} M)^\dagger$ are orthogonal projectors.
\end{proof}

% \textcolor{blue}{... not completely... Intuition: One can think of the projector on the LHS of \cref{eq:proj_id_PM_with_Y} as the projector $I-MM^\dagger$ restricted to the range of $\orthproj$. Since we assume the range of $M$ lies inside of that of $\orthproj$, the projector $I-MM^\dagger$ therefore still annihilates $M$ when restricted to the range of $\orthproj$.}

Now we can prove the analogue of~\cref{thm:error-bound}.

\begin{theorem}\label{thm:orthogonal-tt-sketch-bound}
  Suppose that $r_\mu^L < r_\mu^R-1$ for all $\mu$, and that the DRMs defined in \cref{eq:def_Xmu_Ymu} are standard Gaussian. 
  If the sketched matrices $\Psi^L_\mu$ and $\Omega^L_\mu$ in \cref{alg:orth-sketch} have full rank for all $\mu<d$,
  then for any $(\hat r_1,\dots,\hat r_{d-1})$ such that $\hat r_\mu < r_\mu^L-1$, the OTTS approximation $\tilde{\mc T}$ of $\mathcal T$ obtained from \cref{alg:orth-sketch} satisfies 
  \begin{equation}\label{eq:Pyth_error_OTTS}
    \|\tilde{\mc T} - \mathcal T\|^2_F \leq  \sum_{\mu=1}^{d-1}\|\mathcal T^{\leq \mu} - \proj_{\mc T^{\leq \mu}X_\mu,Y_\mu}\mathcal T^{\leq \mu}\|_F^2.
  \end{equation}
  In expectation it also satisfies
  \begin{equation}\label{eq:exp_error_OTTS}
    \E \|\tilde{\mc T} - \mathcal T\|^2_F \leq \left(\sum_{\mu=1}^{d-1}c_\mu'\right)\sum_{k>\hat r_\mu} \sigma_k(\mathcal T^{\leq \mu})^2 \leq \left(\sum_{\mu=1}^{d-1}c_\mu'\right)\|\mathcal T_{\hat{\mathbf r}} - \mathcal T\|^2_F,
  \end{equation}
  where $\mathcal T_{\hat {\mathbf r}}$ is any best TT approximation of $\mathcal T$ of rank $(\hat r_1,\dots,\hat r_{d-1})$ , and $c_\mu'$ is given by
  \begin{equation}
    c'_{\mu} \coloneqq \left(1+\frac{r_\mu^R}{r_\mu^R-r_\mu^L-1}\right)\left(1+\frac{\hat r_\mu}{r_\mu^L-\hat r_\mu -1}\right).
  \end{equation}
\end{theorem}

\begin{proof}
  By construction of the algorithm, we have $C_d = C_{\leq d-1}^\top \mathcal T^{\leq d-1}$. The approximation $\tilde{\mc T}^{\leq d}$ therefore equals $C_{\leq d} = (C_{\leq d-1} \otimes I) C_{d}^L = (C_{\leq d-1} C_{\leq d-1}^\top \otimes I) \mathcal T^{\leq d}$.  Since the cores are left-orthogonal for $\mu < d$, we have that $C_{\leq \mu}$ is an $(n_1\cdots n_\mu)\times r_\mu^L$ matrix with orthonormal columns. Therefore ${\orthproj}_\mu \coloneqq C_{\leq \mu} C_{\leq \mu}^\top$ is an orthogonal projector for $\mu < d$. The approximation error is thus given by 
  \begin{equation}
     \| \mathcal T - \tilde{\mc T}\|^2_F=\|\mathcal T^{\leq d-1}-\mathit{\Pi}_{d-1} \mathcal T^{\leq d-1}\|^2_F.
  \end{equation}
  We will proceed by inductively bounding 
  \begin{equation}\label{eq:ortho-approx-stage-mu}
    \|\mathcal T^{\leq \mu}-\mathit{\Pi}_\mu \mathcal T^{\leq \mu}\|^2_F.
  \end{equation}
  
  Define $M_\mu \coloneqq \mc T^{\leq \mu}X_\mu(Y_\mu^\top \mc T^{\leq \mu}X_\mu)^\dagger$ and set $\mathit{\Pi}_0=1$. We claim  for $\mu=1,\ldots, d-1$ that
  \begin{equation}\label{eq:recursion_orthproj_with_M}
   \mathit{\Pi}_\mu =  (\mathit{\Pi}_{\mu-1}\tensor I)M_\mu \left( (\mathit{\Pi}_{\mu-1}\tensor I)M_\mu\right)^\dagger.
  \end{equation}
  By the nestedness relation of TTs, we have for all $\mu$ that
  \[
   C_{\leq \mu} = (C_{\leq \mu-1} \tensor I)C_\mu^L.
  \]
  Recall that the core $C_\mu$ is obtained as the left orthogonalization of the tall matrix
  \[
   B_\mu^L=\Psi_\mu^L \Omega_\mu^\dagger = (C_{\leq \mu-1}^\top \tensor I)\mc T^{\leq \mu}X_\mu(Y_\mu^\top \mc T^{\leq \mu}X_\mu)^\dagger.
   \]
   Since the matrices $\Psi_\mu^L$ and $\Omega_\mu^\dagger$ have full column rank by assumption, the same holds for $B_\mu^L$. 
  Therefore $\Ran C_\mu^L = \Ran B_\mu^L$ and thus also
  \[
   \Ran \, (C_{\leq \mu-1}^\top \tensor I) C_\mu^L = \Ran \, (C_{\leq \mu-1}^\top \tensor I) B_\mu^L,
  \]
  since $C_{\leq \mu-1}^\top \tensor I$ has full column rank. The claim \cref{eq:recursion_orthproj_with_M} now follows from 
  \begin{align*}
    (C_{\leq \mu-1} \tensor I)B_\mu^L&= (C_{\leq \mu-1} \tensor I)(C_{\leq \mu-1}^\top \tensor I)\mc T^{\leq \mu}X_\mu(Y_\mu^\top \mc T^{\leq \mu}X_\mu)^\dagger =  (\mathit{\Pi}_{\mu-1}\tensor I)M_\mu.
    %&= (\Pi_{\mu-1}\tensor I)\mc T^{\leq \mu}X_\mu(Y_\mu^\top \mc T^{\leq \mu}X_\mu)^\dagger\\
    % &\coloneqq 
  \end{align*}
  
  
%   with $R_\mu$ invertible a.s.
%   is nor
%   that $B_\mu=(C_{\leq \mu-1}^\top \tensor I)\mc T^{\leq \mu}X_\mu(Y_\mu^\top \mc T^{\leq \mu}X_\mu)^\dagger$ denotes the core $C_\mu$ \textit{before} orthogonalization, i.e. $B_\mu = C_\mu R_\mu$, with $R_\mu$ invertible. Therefore 
%   Since $(C_{\leq \mu-1} \tensor I)C_\mu^L$ is a tall $(n_1\cdots n_\mu)\times r_\mu^L$ matrix of full column rank, we can verify
%   \begin{align*}
%     \mathit{\Pi}_\mu &= (C_{\leq \mu-1} \tensor I)C_\mu^L ((C_{\leq \mu-1} \tensor I)C_\mu^L)^\top
%     % &=(C_{\leq \mu-1} \tensor I)C_\mu ((C_{\leq \mu-1} \tensor I)C_\mu)^\dagger\\
%     =(C_{\leq \mu-1} \tensor I)B_\mu^L ((C_{\leq \mu-1} \tensor I)B_\mu^L)^\dagger.
%   \end{align*}
%   Denoting $M_\mu = \mc T^{\leq \mu}X_\mu(Y_\mu^\top \mc T^{\leq \mu}X_\mu)^\dagger$,  observe that 
%   \begin{align*}
%     (C_{\leq \mu-1} \tensor I)B_\mu^L&= (C_{\leq \mu-1} \tensor I)(C_{\leq \mu-1}^\top \tensor I)\mc T^{\leq \mu}X_\mu(Y_\mu^\top \mc T^{\leq \mu}X_\mu)^\dagger =  (\mathit{\Pi}_{\mu-1}\tensor I)M_\mu.
%     %&= (\Pi_{\mu-1}\tensor I)\mc T^{\leq \mu}X_\mu(Y_\mu^\top \mc T^{\leq \mu}X_\mu)^\dagger\\
%     % &\coloneqq 
%   \end{align*}
%   In short $\mathit{\Pi}_\mu =  (\mathit{\Pi}_{\mu-1}\tensor I)M_\mu \left( (\mathit{\Pi}_{\mu-1}\tensor I)M_\mu\right)^\dagger$. 
  
  We can use \cref{eq:recursion_orthproj_with_M} to rewrite \cref{eq:ortho-approx-stage-mu} as
  \begin{equation} \label{eq:OTTS_Pyth_error}
  \begin{aligned}
    \|\mathcal T^{\leq \mu}-&\orthproj_\mu \mathcal T^{\leq \mu}\|_F^2 = \|\mathcal T^{\leq \mu}- (\orthproj_{\mu-1}\tensor I)M_\mu \left( (\orthproj_{\mu-1}\tensor I)M_\mu\right)^\dagger\mathcal T^{\leq \mu}\|_F^2 \\
    % &= \|\mathcal T^{\leq \mu}- (\orthproj_{\mu-1}\tensor I)\mathcal T^{\leq \mu} + (\orthproj_{\mu-1}\tensor I)\mathcal T^{\leq \mu}- (\orthproj_{\mu-1}\tensor I)M_\mu \left( (\orthproj_{\mu-1}\tensor I)M_\mu\right)^\dagger\mathcal T^{\leq \mu}\|^2 \\
    &= \|\mathcal T^{\leq \mu}- (\orthproj_{\mu-1}\tensor I)\mathcal T^{\leq \mu}\|_F^2 + \|(\orthproj_{\mu-1}\tensor I)\mathcal T^{\leq \mu}- (\orthproj_{\mu-1}\tensor I)M_\mu \left( (\orthproj_{\mu-1}\tensor I)M_\mu\right)^\dagger\mathcal T^{\leq \mu}\|_F^2.  
    % &\leq \|\mathcal T^{\leq \mu-1}- \orthproj_{\mu-1} \mathcal T^{\leq \mu-1}\|_F^2 + \|\mathcal T^{\leq \mu}- M_\mu \left( (\orthproj_{\mu-1}\tensor I)M_\mu\right)^\dagger\mathcal T^{\leq \mu}\|_F^2 
  \end{aligned}
  \end{equation}
  In the second step we used the Pythagoras theorem since the matrix of the first term lies in the kernel of the orthogonal projector $\orthproj_{\mu-1}\tensor I$, while the matrix of the second term lies in its image. 
  
  The first term in \cref{eq:OTTS_Pyth_error} equals $\|\mathcal T^{\leq \mu-1}-\orthproj_{\mu-1} \mathcal T^{\leq \mu-1}\|^2_F$. To bound the second term, we use \cref{lem:projector-inequality} with $M=M_\mu$ and $Y=Y_\mu$, so that $M_\mu Y_\mu^\top  = \proj_{\mc T^{\leq \mu}X_\mu,Y_\mu}$. Since $(\orthproj_{\mu-1}\otimes I)M_\mu$ has full column rank, we therefore get
%   Note that since $r_\mu^L<r_\mu^R$, the matrix $M_\mu$ has a.a. full column rank. Therefore, so long as $M_\mu$ is not in the kernel of $\Pi_{\mu-1}\otimes I$ (which happens with probability zero), the product $(\Pi_{\mu-1}\otimes I)M_\mu$ has full column rank. 
  \begin{align*}
    \|(\orthproj_{\mu-1}\tensor I)\mathcal T^{\leq \mu}- (\orthproj_{\mu-1}\tensor I)M_\mu \left( (\orthproj_{\mu-1}\tensor I)M_\mu\right)^\dagger\mathcal T^{\leq \mu}\|_F^2 \leq \|\mathcal T^{\leq \mu} - \proj_{\mc T^{\leq \mu}X_\mu,Y_\mu}\mathcal T^{\leq \mu}\|_F^2.
  \end{align*}
 By induction we then obtain \cref{eq:Pyth_error_OTTS}. 
 Observing that the above term is also the GN approximation error, we get from \cref{eq:OTTS_Pyth_error} and \cref{thm:GN} with $\hat r_\mu < r_\mu^ L -1$ that
  \begin{equation}
    \E\|\mathcal T^{\leq \mu}-\orthproj_\mu \mathcal T^{\leq \mu}\|^2_F \leq \E \|\mathcal T^{\leq \mu-1}-\orthproj_{\mu-1} \mathcal T^{\leq \mu-1}\|^2_F + c_\mu'\sum_{k>\hat r_\mu} \sigma_k(\mathcal T^{\leq \mu})^2.
  \end{equation}
  By induction we then obtain the first inequality in \cref{eq:exp_error_OTTS}. The second inequality in \cref{eq:exp_error_OTTS} follows from \cref{eq:sing_val_lower_bound_best_rank} like in the proof of \cref{thm:error-bound}.
\end{proof}

The assumption in the theorem on the full-rankness of the sketches can be avoided if the cores $C_\mu$ are allowed to have a rank smaller than $r^L_\mu$. This can be done naturally during the orthogonalization of $B_\mu^L$. It would however require that the size of DRM $Y_\mu$ is also adjusted accordingly. 


